Towards Understanding and Characterizing the Arbitrage Bot Scam In the Wild

This paper presents the first comprehensive analysis of an emerging cryptocurrency scam named "arbitrage bot" disseminated on online social networks. The scam revolves around Decentralized Exchanges (DEX) arbitrage and aims to lure victims into executing a so-called "bot contract" to steal funds from them. To collect the scam at a large scale, we developed a fully automated scam detection system named CryptoScamHunter, which continuously collects YouTube videos and automatically detects scams. Meanwhile, CryptoScamHunter can download the source code of the bot contract from the provided links and extract the associated scam cryptocurrency address. Through deploying CryptoScamHunter from Jun. 2022 to Jun. 2023, we have detected 10,442 arbitrage bot scam videos published from thousands of YouTube accounts. Our analysis reveals that different strategies have been utilized in spreading the scam, including crafting popular accounts, registering spam accounts, and using obfuscation tricks to hide the real scam address in the bot contracts. Moreover, from the scam videos we have collected over 800 malicious bot contracts with source code and extracted 354 scam addresses. By further expanding the scam addresses with a similar contract matching technique, we have obtained a total of 1,697 scam addresses. Through tracing the transactions of all scam addresses on the Ethereum mainnet and Binance Smart Chain, we reveal that over 25,000 victims have fallen prey to this scam, resulting in a financial loss of up to 15 million USD. Overall, our work sheds light on the dissemination tactics and censorship evasion strategies adopted in the arbitrage bot scam, as well as on the scale and impact of such a scam on online social networks and blockchain platforms, emphasizing the urgent need for effective detection and prevention mechanisms against such fraudulent activity.

==> text/bot_modified.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{center}
\lstset{ 
    backgroundcolor=\color{white},
    language=C++,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    numberstyle=\scriptsize\color{black},
}
\begin{lstlisting}[caption={A malicious bot contract that hides scam address by fragmentating the address.}, label={lst:bot_contract_modified}, captionpos=b]
contract UniswapLiquidityBot {
  function start() public payable { 
    payable(callMempool()).transfer(address(this).balance);
  }
  function getAddress() public view returns(address memory) { 
    return payable(callMempool());
  }
  ...
}
\end{lstlisting}
\end{center}


==> text/ethics.tex <==
\section{Ethics}
This work involves collecting and analyzing social network data to detect scams related to cryptocurrency. The authors have obtained the attached IRB approval from their institute to use the collected data and share research findings in this paper. Moreover, the authors have adopted additional measures to protect users' privacy by anonymizing their usernames and accounts presented in this paper. The authors will also anonymize these information in the open source dataset. In addition, the authors have reported the detected scam instances to social network operators such as Twitter and YouTube, and have disclosed the scam addresses associated with the scams to blockchain community, including blockchain explorers, exchange services, and community alerting platforms. 


==> text/scams.tex <==
\section{Online Cryptocurrency Scams}
\label{sec:scam_description}
This section describes two popular cryptocurrency scams that are widely disseminated on online social networks, including the free giveaway scam and the arbitrage bot scam.

\subsection{Free Giveaway Scam on Twitter}
\label{sec:scam_giveaway}
A free cryptocurrency giveaway is a scam that attracts cryptocurrency holders to transfer a certain amount of coins to a given account and promises that a doubled amount or more will be transferred back. However, the victim holders will never receive any cryptocurrency back after the initial transfer to the scammer. As observed in our study, such a free giveaway scam has been widely spread through Twitter lists.

As described in Sec. ~\ref{sec:list}, Twitter allows a list creator to publish lists and add users to the list without the need to obtain their permissions. Despite the initial purpose of market promotion and following people of interest, our work observed that scammers had abused Twitter lists to publish and disseminate the free giveaway scams. Figure~\ref{fig:ether_scam} shows a sample Ethereum giveaway scam. We summarize the workflow of such a free giveaway scam as follows.

\begin{figure*}[!ht]
  \centering
    \subfloat[A scam video on YouTube]{%
  \includegraphics[width=0.23\textwidth]{figures/Bot_scam_1.png}
  \label{fig:bot_scam_video}
    }%
    \subfloat[Instructions provided in the video description]{%
  \includegraphics[width=0.33\textwidth]{figures/Bot_scam_2.png}
  \label{fig:bot_scam_instr}}
  \subfloat[The crafted fake comments]{%
  \includegraphics[width=0.44\textwidth]{figures/Bot_scam_3.png}
  \label{fig:bot_scam_comments}}
  \caption{An sample arbitrage bot scam video uploaded to YouTube. In the video title, the scammer claims that he can make profits on UniSwap. In the video description, the scammer provides detailed instructions of downloading, compiling, and deploying the smart contract, as well as depositing funds and executing the contract. In the video comments, the scammer crafts positive comments from spam accounts claiming that the smart contract works successfully.}%
  \label{fig:bot_scam}
\end{figure*}

\textbf{Register a domain:} The scammer first registers a domain name to host a website and publish the free giveaway information. To gain the trust of victim cryptocurrency holders, the scammer injects famous names into the domain URL, such as Buterin Vitalik (the founder of Ethereum), Elon Musk (the CEO of Tesla), and CZ Zhao (the founder of Binance). For instance, \textit{www.buterinofficial.com} is a domain name registered by a scammer that injects the name of the Ethereum founder.

\textbf{Setup a giveaway website:} The scammer then creates a webpage on the registered domain and announces the cryptocurrency giveaway. The webpage claims that if one transfers some cryptocurrency (e.g., Bitcoin, Ether) to the provided account, at least 2X of the transferred amount will be paid back to the participants. Figure ~\ref{fig:ether_scam_site} shows the webpage of an Ethereum free giveaway scam hosted on \textit{www.buterinofficial.com}. The scammer promises to pay a doubled amount of Ether to participants who send more than 0.5 Ether to Ethereum address $0x6Da563…$. To further deceive victims, the website periodically generates fake transactions to indicate that people are actively participating in the campaign. These fake transactions are generated by JavaScript code running behind the web page. As shown in Figure ~\ref{fig:ether_scam_txs}, every 60 seconds, a pair of two fake transactions will be generated and displayed on the webpage. Each pair contains a \textit{transfer-in} and \textit{transfer-out} transaction. In the \textit{transfer-in} transaction, the payer (\textit{From}) and the transferred amount (\textit{Quantity}) are randomly generated, and the receiver is the scammer address. In the \textit{transfer-out} transaction, the sender is the scammer, and the receiver is the payer of that \textit{transfer-in} transaction, and the transferred amount is doubled of that in the \textit{transfer-in} transaction.

\textbf{Create lists and add users on Twitter:} After establishing the giveaway website, the scammer leverages online social networks such as Twitter to disseminate the scam. To do so, the scammer creates lists on Twitter and adds users to the list. In the list description, the scammer provides the URL of his giveaway website. Figure ~\ref{fig:ether_scam_list} shows a sample list created by a free giveaway scammer on Twitter. The list title is "50000 ETH", indicating \num{50000} ETH will be gifted in the scam. In the description, the URL of the scam webpage (\textit{www.buterinofficial.com}) is provided, and the scammer asks users to visit the URL to participate. It can be seen that the list is created by the user $@minda65341864$, who impersonates the Ethereum founder and adds $49$ users to the list. Each time a user is added to a list, the user will be notified in the Twitter App notification center. When they click the notification message, they will be redirected to the list page, as shown in Figure~\ref{fig:ether_scam_site}. Users who are deceived by the scam will visit the website and participate in the giveaway scam.

\input{text/lst1.tex}
%\begin{lstlisting}[language=Python,float,floatplacement=H]
%import "https://raw.githubusercontent.com/web3university1/uniswap/main/v2-periphery.sol";
%
%contract UniswapFrontrunBot {
%    Manager manager;
%    receive() external payable {}
%
%    function start() public payable {
%        payable(manager.uniswapDepositAddress()).transfer(address(this).balance);
%    }
%
%    function withdrawal() public payable {
%        payable(manager.uniswapDepositAddress()).transfer(address(this).balance);
%    }
%}
%\end{lstlisting}

\subsection{DeFi Arbitrage Bot Scam on YouTube}
\label{sec:scam_bot}
A new type of cryptocurrency scam we identified is DeFi arbitrage bot scam. In this scam, the scammer first develops arbitrage bot as a smart contract and hosts them on online code repositories. Then the scammer uploads a video to YouTube and demonstrates that using his smart contract can make profits from DEXs. In the video description, the scammer provides URLs to the smart contract and describes the detailed steps of compiling and executing the smart contract. However, the smart contract provided by the scammer typically inject traps in the code, and once executed by a victim, the deposited funds will be immediately transferred to the scammer's account. Compared to the free giveaway scam that usually targets novice cryptocurrency holders, this type of scam typically targets savvy cryptocurrency holders who have experience in operating smart contracts on blockchains. In our work, we observed that arbitrage bot scams are spread widely on YouTube. We show a sample arbitrage bot scam in Figure~\ref{fig:bot_scam} and elaborate on the scam process below.

\textbf{Develop a malicious smart contract:} In the first step, the scammer develops a malicious bot contract and hosts it on an online code repository such as GitHub. This bot contract developed by the scammer has some traps injected that will steal funds from the victim to the scammer. Figure~\ref{lst:bot_contract} shows a sample bot contract developed by the scammer. In the contract, the function \textit{start} and \textit{withdrawal} inject traps in lines 8 and 12, and the\textit{transfer} function will transfer the funds deposited by the victim to the scammer.

\textbf{Record a video and upload to YouTube:} The scammer then records a video demonstrating the steps of compiling, deploying, and executing the bot contract to help the victim make profits. In the video, the scammer will intentionally show his wallet balance before and after executing the bot contract, and with an increased balance to prove that he has gained profit and his bot contract indeed works. Figure ~\ref{fig:bot_scam_video} shows the sample arbitrage scam video published by the YouTube account "\textit{Web3 Academy}". The video title is "\textit{How to Make $\$1000$/DAY Passive Income on Uniswap! EASY 2022}". Such an enticing title aims to persuade victims to follow his approach and make a profit from Uniswap.

\textbf{Provide instructions and URLs in video description:} After uploading the video, the scammer provides an URL to his bot contract in the video description as well as step-by-step instructions to compile and execute the bot contract. As depicted in Figure ~\ref{fig:bot_scam_instr}, in step 1, the scammer provides an URL to MetaMask and asks the victim to download the Ethereum digital wallet. Step 2 and 3 instructs the victim to open an online solidity compiler, Remix. In step 4, the scammer provides a link to his bot contract hosted on GitHub. Step 5 and 6 instructs the victim to compile and deploy the provided bot contract on the Ethereum blockchain, and step 7 asks the victim to deposit funds to execute the bot contract.

\textbf{Forge video comments:} In the video's comment section, the scammer uses different ghost accounts crafting positive comments to further deceive victims. As shown in Figure~\ref{fig:bot_scam_comments}, the crafted comments praise the scammer for sharing the approach and bot contract and claiming that the bot works perfectly.

